A Phenomenological Study of WIMP Models

In this thesis, we investigate various possibilities of Weakly Interacting Massive Particle (WIMP) dark matter (DM) and their implications. These possibilities are important because they challenge the viability of WIMP DM in light of tight constraints from experiments such as direct detection. We begin by analyzing a fermion dark matter possibility with an axion-like particle (ALP) portal. We consider theoretical and experimental limits related to neutrino and ALP data within a certain mass range, and we find the allowed parameter space. This possibility resolves the problem of the lack of direct detection of WIMP DM through the ALP portal. Furthermore, we examine the limits on photon signals from HESS and Fermi-LAT data. Next, we look at a two-component scalar and fermion dark matter possibility, following a similar approach to our previous work. This simple possibility requires only a few additional fields and symmetries to explain neutrino mass and dark matter candidates. By finding parameter space that satisfies various bounds, such as relic density, direct detection, and invisible Higgs width, we show that both scalar and fermion particles can serve as DM. This possibility is consistent and offers a rich spectrum of phenomenology that can be tested through collider-based experiments. In our final work, we removie the extra Z2 symmetry and added a new pseudoscalar particle in our two compoent model. We test this pseudoscalar particle against multiple DM and non-DM related bounds, including DM lifetime bound, Planck bound, direct-detection limits from various target materials, and invisible Higgs width. The possibility exhibits a significant parameter space for our pseudoscalar DM while being in agreement with theoretical and experimental limits.

==> pagestyle1.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \cleardoublepage
% \pagestyle{plain}
% \pagestyle{fancy}
% \renewcommand{\chaptermark}[1]{ \markboth{#1}{} }
% %\renewcommand{\sectionmark}[1]{ \markright{#1}{} }
% 
% \fancyhf{}
% \fancyhead[LE,RO]{\thepage}
% \fancyhead[RE]{\textit{ \nouppercase{\leftmark}} }
% \fancyhead[LO]{\textit{ \nouppercase{\rightmark}} }
% 
% \fancypagestyle{plain}{ %
%   \fancyhf{} % remove everything
%   \renewcommand{\headrulewidth}{0pt} % remove lines as well
%   \renewcommand{\footrulewidth}{0pt}
% }


%%%%%%%%%%%%%%  Page style %%%%%%%%%%%%%%%%%%%%
% \definecolor{armygreen}{rgb}{0.29, 0.33, 0.13}


\definecolor{headercolor}{gray}{0.55} % chapter numbers will be semi transparent .5 .55 .6 .0
%%%
%%% fancy header options
%%%
% 
% % redefine the plain style
% \fancypagestyle{plain}{%
% \fancyhf{} % clear all header and footer fields 
% % \fancyfoot[C]{\fontfamily{ppl}\selectfont \small\bfseries \thepage} % except the center 
% \renewcommand{\headrulewidth}{0.3pt} 
% \renewcommand{\footrulewidth}{0pt}}
%
% define the style fancy
\pagestyle{fancy}
%\renewcommand{\chaptermark}[1]{\markboth{\thechapter.\ \ #1}{}}
\renewcommand{\chaptermark}[1]{\markboth{#1}{}}
\renewcommand{\sectionmark}[1]{\markboth{#1}{}}
\fancyhf{}
\fancyhead[LE,RO]{\fontfamily{ppl}\selectfont \small\bfseries\thepage}
\fancyhead[LO]{\fontfamily{ppl}\selectfont \small\bfseries\nouppercase{\color{headercolor}\rightmark}}
\fancyhead[RE]{\fontfamily{ppl}\selectfont \small\bfseries\nouppercase{\color{headercolor}\leftmark}}
\renewcommand{\headrulewidth}{0.3pt}
\renewcommand{\footrulewidth}{0pt}
\addtolength{\headheight}{0.4pt} % leave space for the line
\renewcommand{\headrule}{{\color{headercolor} \hrule width\headwidth height\headrulewidth \vskip-\headrulewidth}}

% removes headings from empty pages
% \usepackage{emptypage}

\definecolor{halfgray}{gray}{0.55} % chapter numbers will be semi transparent .5 .55 .6 .0
\newfont{\chapNumFont}{eurb10 scaled 7000}
\newfont{\chapTitFont}{pplr9d}
% 
\titleformat{\chapter}[block]%
{\Huge}{\raggedleft{\color{halfgray}\chapNumFont\thechapter}}{20pt}%
{\raggedright{\fontfamily{ppl}\selectfont #1}}
%


